LLM4Decompile: Decompiling Binary Code with Large Language Models

Decompilation aims to convert binary code to high-level source code, but traditional tools like Ghidra often produce results that are difficult to read and execute. Motivated by the advancements in Large Language Models (LLMs), we propose LLM4Decompile, the first and largest open-source LLM series (1.3B to 33B) trained to decompile binary code. We optimize the LLM training process and introduce the LLM4Decompile-End models to decompile binary directly. The resulting models significantly outperform GPT-4o and Ghidra on the HumanEval and ExeBench benchmarks by over 100% in terms of re-executability rate. Additionally, we improve the standard refinement approach to fine-tune the LLM4Decompile-Ref models, enabling them to effectively refine the decompiled code from Ghidra and achieve a further 16.2% improvement over the LLM4Decompile-End. LLM4Decompile demonstrates the potential of LLMs to revolutionize binary code decompilation, delivering remarkable improvements in readability and executability while complementing conventional tools for optimal results. Our code, dataset, and models are released at https://github.com/albertan017/LLM4Decompile

==> figure/case.tex <==
\begin{figure}[t]
  \centering
  \includegraphics[width=0.95\linewidth]{img/case.pdf}
  \caption{Limitation to use BLEU and Edit Similarity for evaluating decompilation results.}
  \label{fig:case}
\end{figure}

==> figure/pipeline.tex <==
\begin{figure}[t]
  \centering
  \includegraphics[width=0.95\linewidth]{img/pipeline.pdf}
  \caption{Pipeline to evaluate the decompilation.}
  \label{fig:pipeline}
\end{figure}

==> figure/train.tex <==
\begin{figure}[t]
  \centering
  \includegraphics[width=0.8\linewidth]{img/train.pdf}
  \caption{Training objectives}
  \label{fig:train}
\end{figure}

==> sections/legacy_CEnd.tex <==
\section{End2End-Decompile}\label{sec:end}
In this section, we access the performance for the \deend{} approach. We first describe the \deend{} framework, present details for the experimental setups, and discuss the results.

\subsection{The End2End-Decompile Framework}
\begin{figure}[t]
  \centering
  \includegraphics[width=0.9\linewidth]{img/compile-decompile.pdf}
  \caption{\deend{} framework. The source code (SRC) is compiled to binary, disassembled to assembly instructions (ASM), and decompiled by LLM4Decompile to generate SRC'. Loss is computed between SRC and SRC' for training.}
  \label{fig:compile}
\end{figure}
Figure~\ref{fig:compile} illustrates the \deend{} framework, starting from compilation to decompilation processes. During compilation, the Preprocessor processes the source code (SRC) to eliminate comments and expand macros or includes. The cleaned code is then forwarded to the Compiler, which converts it into assembly code (ASM). This ASM is transformed into binary code (0s and 1s) by the Assembler. The Linker finalizes the process by linking function calls to create an executable file. Decompilation, on the other hand, involves converting binary code back into a source file. LLMs, being trained on text, lack the ability to process binary data directly. Therefore, binaries must be disassembled into assembly language (ASM) first. It should be noted that binary and disassembled ASM are equivalent, they can be interconverted, and thus we refer to them interchangeably. Finally, the loss is computed between the decompiled and the source code to guide the training of the LLM.

\subsection{Experimental Setups}

\paragraph{Training Data.}\label{sec:config}
We construct asm-source pairs based on Exebench~\cite{exebench}, which is a public collection of four million compilable C files, where we only consider the decompilation of GCC~\cite{gcc_compile} compiled C under x86 Linux platform.
In the real deployment, programmers will choose different compiler optimization flags to optimize the execution performance. 
It involves techniques like eliminating redundant instructions, better register allocation, loop transformations, etc~\cite{compiler_opt}. 
The key optimization levels are: \textbf{O0} (default, no optimization) to \textbf{O3} (aggressive optimizations, compilation time consuming). We compile the source code into all four stages, i.e., O0, O1, O2, and O3, and pair each of them with the source code. 
To train the model, we use the following template: \texttt{\# This is the assembly code: [ASM code] \# What is the source code? [source code]}, where \texttt{[ASM code]} corresponds to the disassembled assembly code from the binary, and \texttt{[source code]} is the original C function. Note that the choice of template does not impact the performance, since we fine-tune the model to produce the source code.

It's significantly easier to extract C code that is compilable but not linkable——the code can be compiled into a binary object file but not into an executable due to missing links in function calls\cite{anghabench,exebench}. Such binary object code will closely resemble its executable version except it lacks linked addresses for external symbols. In the Exebench dataset, 4.3 million codes are compilable, yet only 446 thousand functions are executable in our tests. To optimize the use of this dataset while maintaining practical relevance, we initially use the 4.3 million compilable codes to fine-tune our model. Subsequently, we enhance the model further using the executable code to develop LLM4Decompile-End. We conduct an ablation study on the dataset in Section~\ref{sec:ablation}.
To refine our training set, we follow the guidelines of StarCoder~\cite{starcoder} by computing MinHash~\cite{minhash} for the code and utilizing Locally Sensitive Hashing (LSH) to remove duplicates. We also excluded samples that were less than 10 tokens. Consequently, our refined compilable training dataset includes 7.2 million samples, containing roughly 7 billion tokens, executable training dataset includes 1.6 million samples, containing roughly 572 million tokens.

\paragraph{Evaluation Benchmark and Metrics.}
To evaluate the models, we introduce HumanEval~\cite{humaneval} and Exebench~\cite{exebench} benchmarks. HumanEval is the leading benchmark for code generation assessment and includes 164 programming challenges with accompanying Python solutions and assertions. We converted these Python solutions and assertions into C, making sure that they compile with the GCC compiler using standard C libraries and pass all the assertions, and name it HumanEval-Decompile. ExeBench consists of 5000 real-world C functions taken from GitHub with IO examples. 
Note that the HumanEval-Decompile consists of individual functions that depend only on the standard C library. In contrast, ExeBench includes functions extracted from real-world projects with user-defined structures and functions.

As for the evaluation metrics, we follow previous work to calculate the re-executability rate~\cite{slade,refine_decompile}. During evaluation, the C source code is first compiled into a binary, then disassembled into assembly code, and fed into the decompilation system to be reconstructed back into C code. This decompiled C code is then combined with the assertions to check if it can successfully execute and pass those assertions. 

\paragraph{Model Configurations.}
Our LLM4Decompile uses the same architecture as DeepSeek-Coder~\cite{deepseekcoder} and we initialize our model with the corresponding DeepSeek-Coder checkpoints. We employ Sequence-to-sequence prediction (S2S), which is the training objective adopted in most neural machine translation models that aim to predict the output given the input sequence. 
As depicted in Equation \ref{eq2}, it minimizes the negative log probability for the source code tokens $x_i,...,x_j$:
\begin{equation}
    \mathcal L = -\sum_i \log P_i (x_i,...,x_j|x_1,...,x_{i-1}; \theta)
    \label{eq2}
\end{equation}
where the loss is calculated only for the output sequence $x_i...x_j$, or the source code. We also explore other creative training strategies and frameworks, the results are discussed in \textbf{Appendix~\ref{sec:appen_train}}.




\input{table/main_results}
\input{table/ablation_train}




\paragraph{Baselines.}
We selected two key baselines for comparison. First, GPT-4o~\cite{gpt4} represents the most capable LLMs, providing an upper bound on LLM performance. As one of the most powerful language models, GPT-4 significantly surpasses previous LLMs across modalities. Second, \textbf{DeepSeek-Coder}~\cite{deepseekcoder} is selected as the current SOTA open-source Code LLM. It represents the forefront of publicly available models specifically tailored for coding tasks. While recent work Slade~\cite{slade} fine-tunes language model for decompilation, it relies on intermediate compiler outputs, specifically, the *.s file. In practice, however, such intermediate files are rarely released by developers. Therefore, we focus on a more realistic approach, and consider decompilation only from the binaries, for further discussions please refer to Appendix~\ref{sec:appen_exe}.

\paragraph{Implementation.}\label{sec:implement}
We use the DeepSeek-Coder models obtained from Hugging Face~\cite{huggingface}. For 1.3B and 6.7B models, we set a $batch\:size=2048$ and $learning\;rate=2e{-}5$ and train the models with the AdamW optimizer~\cite{adamw} for 2 epochs (15B tokens). Experiments are performed on NVIDIA A100-80GB GPU clusters. Fine-tune the 1.3B and 6.7B LLM4Decompile-End take 12 and 61 days on $8 \times A100$ respectively. Limited by the resources, for the 33B model we only train for 200M tokens which takes 30 days. During the evaluation, we use the \textit{vllm} framework~\cite{kwon2023efficient} to accelerate the generation process. We employ greedy decoding and averaged results of 5 runs to minimize randomness in the generated output.

\subsection{Experimental Results}\label{sec:results}

\paragraph{Main Results.}
Table~\ref{table:main_results} presents the re-executability rate under different optimization states for our studied models. Initially, the base version of DeepSeek-Coder-33B was unable to accurately decompile binaries. It could generate code that seemed correct but failed to retain the original program semantics. GPT-4o shows notable decompilation skills; it was able to decompile non-optimized (O0) code with a success rate of 30.5\%, though the rate significantly decreased to about 11\% for optimized codes (O1-O3).
The LLM4Decompile-End models, on the other hand, demonstrated excellent decompilation abilities. The 6.7B version successfully decompiles and on average retains the program semantics in 45.4\% of cases, whereas the 1.3B version has a success rate of 27.3\%. This improvement underscores the advantages of using larger models to capture a program's semantics more effectively.
While attempting to fine-tune the 33B model, we encountered substantial challenges related to the high communication loads, which significantly slowed the training process and restricted us to using only 150M tokens (Section~\ref{sec:implement}). Despite this limitation, the 33B model still outperforms the 1.3B model, reaffirming the importance of model scaling.

\paragraph{Ablation Study.}\label{sec:ablation}
As discussed in Section~\ref{sec:config}, our training data comprises two distinct sets: 4 million compilable functions (non-executable) and 400,000 executable functions. We conducted an ablation study using these datasets, and the results are displayed in Table~\ref{table:ablation_train}. Here, ``Compilable'' denotes the model trained solely on compilable data, while ``Executable'' indicates models trained exclusively on executable data. Notably, the binary object from compilable functions lacks links to function calls, which is similar in text distribution to the HumanEval-Decompile data, consisting of single functions dependent only on standard C libraries. Consequently, the model trained only on compilable data successfully decompiled 37.5\% of HumanEval-Decompile functions, but only 4.7\% on ExeBench, which features real functions with extensive user-defined function references. On the other hand, the model trained solely on executable data achieved a 26.7\% re-executability rate on the ExeBench test set but faced challenges with single functions, with only a 23.8\% success rate on HumanEval-Decompile due to the smaller size of the training corpus. Therefore, training with the expansive compilable data set provides fundamental decompilation knowledge, and further refinement on this well-informed base yielding a model that performs optimally on average. We have also explored other creative training strategies and frameworks, please refer to discussions in \textbf{Appendix~\ref{sec:appen_train}}.


\paragraph{Further Analyses.}
Figure~\ref{fig:length} illustrates that the re-executability rate decreases as the input length increases, and there is a marked decline in performance at higher levels of code optimization, highlighting the difficulties in decompiling long and highly optimized sequences. Importantly, the performance difference between the 1.3B and 6.7B models showcased in the figure emphasizes the advantages of larger models in such tasks. Larger models, with their expanded computational resources and deeper learning capabilities, are inherently better at resolving the challenges posed by complex decompilations.

The error analysis presented in Figure~\ref{fig:error} for LLM4Decompile-End-6.7B indicates that logical errors are prevalent in the HumanEval-Decompile scenarios, with 64\% of errors due to assertions that the decompiled codes do not pass. In the ExeBench dataset, which features real functions with user-defined structures and types, the major challenges are related to reclaiming these user-specific components. Where 50\% of the errors come from undeclared functions, and 28\% from improper use of structures. Given that these user-defined details are typically lost during the compilation process, reconstructing them can be particularly challenging. Integrating techniques like Retrieval Augmented Generation might supplement the decompilation process with necessary external information.
\begin{figure}[t]
  \centering
  \includegraphics[width=0.8\linewidth]{img/length_test.pdf}
  \caption{Re-executability rate with the growth of input length. 6.7B model is more robust against input length.}
  \label{fig:length}
\end{figure}

\begin{figure}[t]
  \centering
  \includegraphics[width=0.85\linewidth]{img/error.pdf}
  \caption{Types of errors identified in the two benchmarks: LLM4Decomile-End-6.7B faces issues with logical errors in HumanEval-Decompile and user-defined components in Exebench. }
  \label{fig:error}
\end{figure}

==> sections/legacy_DRef.tex <==
\section{Refined-Decompile}
In the previous section, we have demonstrated the potential of using LLMs alone (\deend{}) for decompiling binary code. This section extends that exploration by evaluating the effectiveness of the traditional open-source decompilation tool, \ghidra{}, and preliminarily investigating how it can be enhanced through integration with LLMs (\derefine{}). 
Note that we focus on refining the whole outputs, which is a more general stretagey compared to not just recovers the names or types~\cite{decompile_name,decompile_name2}.
We begin by detailing the process of gathering training data, followed by descriptions of our experimental setups, and conclude with an analysis of the experimental outcomes.

\subsection{The Refined-Decompile Framework}
\begin{figure}[t]
  \centering
  \includegraphics[width=0.9\linewidth]{img/decompile-refine.pdf}
  \caption{\derefine{} framework. It differs from \deend{} (Figure~\ref{fig:compile}) only in the LLM's input, which is pseudo-code decompiled from Ghidra.}
  \label{fig:refine}
\end{figure}
The \derefine{} method is shown in Figure~\ref{fig:refine}. This approach differs from that in Figure~\ref{fig:compile} only in terms of the LLM's input, which in the case of \derefine{} comes from Ghidra's decompilation output. Specifically, Ghidra is used to decompile the binary, and then the LLM is fine-tuned to enhance Ghidra's output. While Ghidra produces high-level pseudo-code that may suffer from readability issues and syntax errors, it effectively preserves the underlying logic. Refining this pseudo-code significantly mitigates the challenges associated with understanding the original logic.

\input{table/bleu_run}

\subsection{Experimental Dataset}\label{sec:refine-data}
The training data is constructed using ExeBench, with Ghidra Headless employed to decompile the binary file. Due to constraints in computational resources, only 400K functions each with optimization levels from O0 to O3 (1.6M samples, 1.6B tokens) are used for training and the evaluation is conducted on HumanEval-Decompile. The model is trained using the same template described in Section~\ref{sec:config}. In addition, followed Nova~\cite{btc,slade}, we access the readability of decompiled results in terms of Edit Similarity score.


\begin{figure}[h]
  \centering
  \includegraphics[width=0.98\linewidth]{img/read_case.pdf}
  \caption{Decompilation results of different approaches. GPT-4o outputs are plausible yet incorrect, and Ghidra's pseudo-code is notably less readable. GPT refined Ghidra result (Ghidra+GPT-4o) marginally enhances readability but fails to correctly render \texttt{for} loops and array indexing. Conversely, LLM4Decompile-End and LLM4Decompile-Ref produce more accurate and comprehensible outputs. }
  \label{fig:read_case}
\end{figure}
\subsection{Experimental Setups}
Configuration settings for the model are consistent with those in Section~\ref{sec:end}. For evaluation, we first access the re-executability rate of Ghidra to establish a baseline. Subsequently, GPT-4o is used to enhance Ghidra's decompilation results with the prompt, \texttt{Generate linux compilable C/C++ code of the main and other functions in the supplied snippet without using goto, fix any missing headers. Do not explain anything.}, following DecGPT~\cite{refine_decompile}. Finally, the LLM4Decompile-Ref model is trained using the dataset mentioned in Section~\ref{sec:refine-data} to refine the Ghidra's output. All experiments are conducted using eight NVIDIA A100-80GB GPUs. For the 1.3B, 6.7B models, the fine-tuning process involves 3.2B tokens in 2 epochs, and requires 1, and 6 days respectively. Limited by the resource, for 33B model we only train for 150M tokens and takes 24 days.




\input{table/obfuscation}




\subsection{Experiment Results}

The results for the baselines and \derefine{} approaches are summarized in Table~\ref{table:bleu_run}. For the pseudo-code decompiled by Ghidra, which is not optimized for re-execution, only an average of 20.1\% of them pass the test cases. GPT-4o assists in refining this pseudo-code and enhancing its quality. The LLM4Decompile-Ref models offer substantial improvements over Ghidra's outputs, with the 6.7B model yielding a 160\% increase in re-executability. Similar to the discussion in Section~\ref{sec:results}, the 33B model outperforms the 1.3B model even though it used considerably less training data. And it achieves performance that is only 3.6\% below the 6.7B model, which benefited from ten times more data. When compared to LLM4Decompile-End-6.7B, the LLM4Decompile-Ref-6.7B model, though trained on just 10\% of the data in LLM4Decompile-Ref models, shows a 16.2\% performance increase, suggesting a greater potential for the \derefine{} approach. 

An analysis of readability across different methods is also conducted, the samples are presented in Figure~\ref{fig:read_case}. For text similarity, all decompiled outputs diverge from the original source code, primarily because the compilation process removes variable names and optimizes the logic structure. GPT-4o hallucinates plausible but incorrect outputs. Ghidra, as mentioned in the Introduction, generates pseudo-code that is particularly less readable and shows the least text similarity to the original code. With refinement from GPT (Ghidra+GPT-4o), there is a marginal improvement in readability. GPT assists in refining type errors like \texttt{undefined4} and \texttt{ulong}, however, it struggles to accurately reconstruct \texttt{for} loops and array indexing. In contrast, both LLM4Decompile-End and LLM4Decompile-Ref generate outputs that are more aligned with the format of the source code and easier to comprehend. To summarize, domain-specific fine-tuning is crucial for enhancing re-executability and readability of decompilation outputs.

==> sections/legacy_DSetup.tex <==
\section{Experiment Setups}
% \subsection{Decompile-Eval Benchmark}
% We introduce HumanEval~\cite{humaneval} and Exebench~\cite{exebench} as the evaluation benchmark. HumanEval is the leading benchmark for code generation assessment and includes 164 programming challenges with accompanying Python solutions and assertions. We converted these Python solutions and assertions into C, making sure that they compile with the GCC compiler using standard C libraries and pass all the original assertions.

% In our evaluation process (Figure~\ref{fig:pipeline}), the C source code is first compiled into a binary, then disassembled into assembly code, and finally fed into the decompilation system to be reconstructed back into C source code. This regenerated C code is compiled with GCC to test re-compilability and combined with the original assertions to check if it can successfully execute and pass those assertions. 


% Currently, there appears to be no benchmark for decompilation evaluation that considers whether code can be recompiled or executed correctly. When assessing decompilation model performance, researchers rely on metrics that measure N-gram similarity (such as BLEU or CodeBLEU) or edit similarity (ES). However, these metrics, commonly used in machine translation and text generation, fail to adapt to the evaluation of programming languages. 

% Programming languages are highly structured and logical, insensitive to the naming of functions and variables, yet very sensitive to the flow of data and logic. Changing variable or function names does not affect the meaning of a program, but a single logical error can alter its entire function and purpose.
% As illustrated in Figure~\ref{fig:case}, the use of BLEU and ES in evaluating code similarity is problematic. 
% For $src_1$, the variation from the original $src$ is confined to type conversion of variable $num$, which leads to high BLEU and ES scores. However, this alteration completely changes the intent of the code. Similarly, $src_2$ achieves high BLEU and ES scores, yet the semantics of the function are lost. Conversely, $src_3$ undergoes normalization of function and variable names, causing no semantic shift yet scoring zero in BLEU against the original code. The example of $src_4$ is more extreme: if the program logic is broken down into multiple lines, the ES drops to 41.4\%, falsely indicating a low similarity. However, during compilation, names are typically standardized by the compiler, and source code is often broken down into basic operations depending on optimization. For this reason, the ability to recompile and execute the code is far more indicative than N-gram or edit similarity for evaluating decompilation efficacy.

% \input{figure/case}

% To address the gap in decompilation assessment, we introduce Decompile-Eval, the first benchmark to evaluate the re-compilability and re-executability of decompilation systems. This benchmark is derived from HumanEval~\cite{humaneval}, which is the leading benchmark for code generation assessment and includes 164 programming challenges with accompanying Python solutions and assertions. We converted these Python solutions and assertions into C, making sure that they compile with the GCC compiler using standard C libraries and pass all the original assertions. In our evaluation process (Figure~\ref{fig:pipeline}), the C source code is first compiled into a binary, then disassembled into assembly code, and finally fed into the decompilation system to be reconstructed back into C source code. This regenerated C code is compiled with GCC to test re-compilability and combined with the original assertions to check if it can successfully execute and pass those assertions. 
% Re-compilability and re-executability serve as critical indicators in validating the effectiveness of a decompilation process. When decompiled code can be recompiled, it provides strong evidence of syntactic integrity. It ensures that the decompiled code is not just readable, but also adheres to the structural and syntactical standards expected by the compiler. 
% However, syntax alone does not guarantee semantic equivalence to the original pre-compiled program. Re-executability provides this critical measure of semantic correctness. By re-compiling the decompiled output and running the test cases, we assess if the decompilation preserved the program logic and behavior.
% Together, re-compilability and re-executability indicate syntax recovery and semantic preservation---both essential for usable and robust decompilation.

% In alignment with established evaluation practices, following Slade~\cite{slade}, we partition 1000 samples from the AnghaBench into a test set. We then utilize BLEU and ES as our primary metrics for assessment.

% \subsection{Baselines}
% To benchmark against SOTA decompilers, we selected two key baselines. First, \textbf{GPT-4} represents the most capable LLMs, providing an upper bound on LLM performance. As one of the largest language models, GPT-4 significantly surpasses previous LLMs across modalities. Second, \textbf{DeepSeek-Coder} is selected as the current SOTA open-source Code LLM. It represents the forefront of publicly available models specifically tailored for coding tasks. While recent academic works like BTC~\cite{btc} and Slade~\cite{slade} showcase LLMs for decompilation, these models present significant integration challenges, such as complex pre-processing settings, non-standardized tokenizer/model loading, and necessitating significant effort to modify and adapt them.
% We thus selected GPT-4 and DeepSeek-Coder as representative cutting-edge and open-source baselines accessible for evaluation.

% \subsection{Implementation}
% We use the Python implementation of the DeepSeek-Coder models (1.3B, 6.7B, and 33B) obtained on Hugging Face~\cite{huggingface}. We set a global $batch\:size=2048$ and $learning\;rate=2e{-}5$ and train the models with the AdamW optimizer~\cite{adamw} for 2 epochs. During the evaluation, we set the $max\_new\_tokens$ to 512. To ensure fairness in the analysis of time and space complexity, all experiments are performed on a cluster equipped with 8 NVIDIA A100-80GB GPUs. 

==> sections/legacy_EResults.tex <==
% \section{Experiment Results}
% \input{table/main_results}
% \input{table/ablation_train}
% \input{table/bleu_run}
% \input{table/obfuscation}
% \subsection{Main Results}
% Table~\ref{table:main_results} presents the primary findings of our study. Initially, the base version of DeepSeek-Coder was unable to accurately decompile binaries. It could generate code that seemed correct and was sometimes compilable but failed to retain the original program semantics. After fine-tuning, the LLM4Decompile models demonstrated a significant improvement in their ability to decompile binaries, with an impressive around 90\% of the code being compilable, signifying a solid understanding of code structure and syntax. As for the ability to execute the code, the 6B version of LLM4Decompile shows a remarkable advantage over the 1B version, 21\% of the decompiled codes from the 6B version successfully capture the semantics of a program and pass all the test cases, while for the 1B version only 10\% can be re-executed. The improvement highlights the benefits of larger model sizes in capturing the semantics of a program. Nonetheless, the increase in model size to 33B yields only a marginal improvement, with an average increase of less than one percentage point in re-executability. This plateau may be due to the challenge of tuning the 33B model.


% \subsection{Ablations}
% As discussed in Section~\ref{sec:config}, our LLM4Decompile model adopts a sequence-to-sequence (S2S) forecasting approach, which outperforms other training techniques for several reasons. In this training methodology, the input—specifically the assembly code is not included in the calculation of the loss function. This allows the model to focus solely on generating accurate output source code, enabling it to better understand the underlying patterns and structures of the decompiled code. In contrast, integrating the assembly code into the training process, as in the next token prediction (NTP) task, encompasses both the input assembly code and the output source code, which can decrease performance by around 4 points, as shown in Table~\ref{table:ablation_train}. The complexity of assembly code is another factor; being inherently complex and low-level, it is harder for the model to learn meaningful patterns when assembly code is included in the training process. By excluding the assembly code from the loss calculation, the S2S approach enables the model to avoid this complexity and concentrate on high-level source code patterns. Although an alternative strategy involves an initial training step with both assembly and C code followed by fine-tuning focused on the translation task (NTP+S2S), this approach still doesn't perform as well as the S2S.

